Sloan Digital Sky Survey IV: Mapping the Milky Way, Nearby Galaxies, and the Distant Universe

We describe the Sloan Digital Sky Survey IV (SDSS-IV), a project encompassing three major spectroscopic programs. The Apache Point Observatory Galactic Evolution Experiment 2 (APOGEE-2) is observing hundreds of thousands of Milky Way stars at high resolution and high signal-to-noise ratio in the near-infrared. The Mapping Nearby Galaxies at Apache Point Observatory (MaNGA) survey is obtaining spatially-resolved spectroscopy for thousands of nearby galaxies (median redshift of z = 0.03). The extended Baryon Oscillation Spectroscopic Survey (eBOSS) is mapping the galaxy, quasar, and neutral gas distributions between redshifts z = 0.6 and 3.5 to constrain cosmology using baryon acoustic oscillations, redshift space distortions, and the shape of the power spectrum. Within eBOSS, we are conducting two major subprograms: the SPectroscopic IDentification of eROSITA Sources (SPIDERS), investigating X-ray AGN and galaxies in X-ray clusters, and the Time Domain Spectroscopic Survey (TDSS), obtaining spectra of variable sources. All programs use the 2.5-meter Sloan Foundation Telescope at Apache Point Observatory; observations there began in Summer 2014. APOGEE-2 also operates a second near-infrared spectrograph at the 2.5-meter du Pont Telescope at Las Campanas Observatory, with observations beginning in early 2017. Observations at both facilities are scheduled to continue through 2020. In keeping with previous SDSS policy, SDSS-IV provides regularly scheduled public data releases; the first one, Data Release 13, was made available in July 2016.

==> authors2astroph <==
#!/usr/bin/env python

import re

afp = open("authors.txt")
author_names = []
for line in afp.readlines():
    words = line.split()
    author_name = " ".join(words[:-1])
		# Note the below messes up \~
    author_name = re.sub('~', ' ', author_name)
    author_names.append(author_name)
afp.close()

afp = open("astroph_authors.txt", "w")
for author_name in author_names:
		afp.write(author_name + ", ")
afp.close()


==> authors2tex <==
#!/usr/bin/env python

import numpy as np

ifp = open("institutions.txt")
institution_addresses = []
institution_codes = []
for line in ifp.readlines():
    words = line.split()
    code = words[0]
    address = " ".join(words[1:])
    institution_address = address  # + " \\label{" + code + "}"
    institution_addresses.append(institution_address)
    institution_codes.append(code)
ifp.close()

afp = open("authors.txt")
author_names = []
author_codes = []
author_codes_all = []
for line in afp.readlines():
    words = line.split()
    author_name = " ".join(words[:-1])
    author_code = words[-1]
    author_names.append(author_name)
    author_codes.append(author_code)
    author_code_list = author_code.split(',')
    for author_code_item in author_code_list:
        author_codes_all.append(author_code_item)
afp.close()

cpos = []
for institution_code in institution_codes:
    cpos.append(author_codes_all.index(institution_code))

isort = np.argsort(np.array(cpos))
addresses = []
codes = []
for indx in isort:
    addresses.append(institution_addresses[indx])
    codes.append(institution_codes[indx])

tfp = open("authors.tex", "w")

tfp.write("\\correspondingauthor")
tfp.write("{Michael R.~Blanton}\n")
tfp.write("\email{michael.blanton@gmail.com}\n")

first_author = True

for author_name, author_code in zip(author_names, author_codes):
    if(first_author):
        orcid = "0000-0003-1641-6222"
        tfp.write("\\author[" + orcid +"]{")
        first_author = False
    else:
        tfp.write("\\author{")
    tfp.write(author_name)
    tfp.write("}\n")
    author_code_list = author_code.split(',')
    for indx, author_code_item in zip(range(len(author_code_list)), author_code_list):
        tfp.write("\\affiliation{")
        tfp.write(addresses[codes.index(author_code_item)])
        tfp.write("}\n")
#tfp.write("}")

#tfp.write("""

#\\setcounter{address}{1}""")
#
#for address, code in zip(addresses, codes):
#    indx = codes.index(code) + 1
#    tfp.write("\\altaffiliation{" + str(indx) + "}")
#    tfp.write("{" + address + "}\n")

tfp.close()


==> makefile <==
#
# Run make -f make.skysub all
#
# $Id: make.skysub 945 2011-03-09 21:29:50Z mb144 $
#
NAME = sdss4

INPUTTEX = intro.tex \
	apo.tex \
	data.tex \
	climate.tex \
	authors.tex \
	apogee2.tex \
	imaging.tex \
	eboss.tex \
	tdss.tex \
	spiders.tex \
	collaboration.tex \
	epo.tex \
	quasar.tex \
	ets.tex \
	lco.tex \
	manga.tex \
	plates.tex \
	project.tex \
	summary.tex \
	acks.tex \
	sdss4.bib \
	sdss4.tex

INPUTFIG = ./eboss_projections.eps \
	./eboss_footprint.pdf \
	./eboss_pie.png \
	./nbar-qso.pdf \
	./eboss-spectra.pdf \
	./sdss4-orgchart.pdf \
	./manga-data.pdf \
	./manga-footprint.pdf \
	./apogee2-footprint.pdf \
	./apogee2-spectra.pdf \
	./apogee2-abundances.pdf 

BIB = ccpp.bib

all: $(NAME).pdf

$(NAME).pdf: $(NAME).tex $(INPUTTEX) $(INPUTFIG)
	pdflatex $(NAME); bibtex $(NAME); pdflatex $(NAME); pdflatex $(NAME)

authors.tex: authors.txt institutions.txt authors2tex
	./authors2tex

clean:
	rm -f *.pdf *.dvi sdss4Notes.bib

fullclean:
	rm -f *.pdf *.log *.dvi *.aux *.bbl *.blg sdss4Notes.bib

test:
	@echo "This should be the correct path to the ccpp.bib file:"
	@echo $(BIB)ccpp.bib

dummy:

